Computing Optimal Equilibria and Mechanisms via Learning in Zero-Sum Extensive-Form Games

We introduce a new approach for computing optimal equilibria via learning in games. It applies to extensive-form settings with any number of players, including mechanism design, information design, and solution concepts such as correlated, communication, and certification equilibria. We observe that optimal equilibria are minimax equilibrium strategies of a player in an extensive-form zero-sum game. This reformulation allows to apply techniques for learning in zero-sum games, yielding the first learning dynamics that converge to optimal equilibria, not only in empirical averages, but also in iterates. We demonstrate the practical scalability and flexibility of our approach by attaining state-of-the-art performance in benchmark tabular games, and by computing an optimal mechanism for a sequential auction design problem using deep reinforcement learning.

==> figures/combined_proof_figures.tex <==
\centering%
\raisebox{-1mm}{\input{figures/staghunt-body}}%
\hfill%
{\input{figures/noncredible-threat}}%
\caption{\textbf{Left:} The counterexample game for \Cref{th:bandit-lower-bound}, for $n=3$. Chance always plays uniformly at random. Infosets are linked by dotted lines (all nodes belonging to the same player are in the same infoset).
    %
    \textbf{Right:} A counterexample game in which Player 2's equilibrium strategy cannot be made weakly dominant solely by adding payments at nodes not reached in equilibrium. Chance plays uniformly at random at the root node.
}%
\label{fig:proof combined}


==> figures/noncredible-threat.tex <==
\newcommand{\util}[2]{{${\color{p1color} \bm{\mathsf{#1}}}$,${\color{p2color} \bm{\mathsf{#2}}}$}}%
\newcommand{\player}[1]{\color{white}\bfseries\sffamily #1}%
\centering%
\tikzset{
    % every path/.style={-stealth},
    infoset1/.style={-, dotted, ultra thick, color=p1color, draw opacity=0.5},
    infoset2/.style={infoset1, color=p2color},
    infoset3/.style={infoset1, color=p3color},
    terminal/.style={},
    s1/.style={}, %ultra thick, color=s1color},
    s2/.style={}, %ultra thick, color=s2color},
}%
\forestset{
    p1/.style={circle, inner sep=1pt, fill=p1color, draw=p1color, font={\player 1}},
    p2/.style={p1, fill=p2color, draw=p2color, font={\player 2}},
    p3/.style={p1, fill=p3color, draw=p3color, font={\player 3}},
    nat/.style={p1, fill=black, draw=black, font={\player C}},
    parent/.style={no edge,tikz={\draw (#1.south) to (!.north); }},
    el/.style={edge label={node[midway, fill=white, inner sep=1pt] {\footnotesize\sf #1}}}
}%
\scalebox{.78}{\begin{forest}
        for tree={l sep=24pt, s sep=5pt}
        [,nat
        [,p2,name=p21,tier=4
            [\util{0}{3}, terminal,el=H]
            [\util{0}{0}, terminal,el=S]
        ]
        [,p1,
        [\util{3}{0}, terminal,el=H]
            [,p2,name=p22,tier=4,el=S
                    [\util{0}{0}, terminal,el=H]
                    [\util{4}{4}, terminal, draw,el=S]]]
        ]
        % \begin{scope}[on background layer]
        \draw[infoset2, bend right=30] (p21) to (p22);
        % \end{scope}
    \end{forest}}%
% \label{fi:nct}

==> figures/staghunt-body.tex <==
\newcommand{\util}[3]{{${\color{p1color} \bm{\mathsf{#1}}}$,${\color{p2color} \bm{\mathsf{#2}}}$,${\color{p3color} \bm{\mathsf{#3}}}$}}%
\newcommand{\player}[1]{\color{white}\bfseries\sffamily #1}%
\centering%
\tikzset{
    % every path/.style={-stealth},
    infoset1/.style={-, dotted, ultra thick, color=p1color, draw opacity=0.5},
    infoset2/.style={infoset1, color=p2color},
    infoset3/.style={infoset1, color=p3color},
    terminal/.style={},
    s1/.style={}, %ultra thick, color=s1color},
    s2/.style={}, %ultra thick, color=s2color},
}%
\forestset{
    p1/.style={circle, inner sep=1pt, fill=p1color, draw=p1color, font={\player 1}},
    p2/.style={p1, fill=p2color, draw=p2color, font={\player 2}},
    p3/.style={p1, fill=p3color, draw=p3color, font={\player 3}},
    nat/.style={p1, fill=black, draw=black, font={\player C}},
    parent/.style={no edge,tikz={\draw (#1.south) to (!.north); }},
    el/.style={edge label={node[midway, fill=white, inner sep=1pt] {\footnotesize\sf #1}}}
}%
\scalebox{0.78}{\begin{forest}
        for tree={l sep=24pt, s sep=5pt}
        [,nat
        [,p1,name=p1,el={$j=1$},tier=4
            [\util{\frac{1}{2}}{0}{0}, terminal, el=H]
            [\util{0}{0}{0}, terminal, el=S]
        ]
        [,p2,name=p2,el={$j=2$},tier=4
            [\util{0}{\frac{1}{2}}{0}, terminal, el=H]
            [\util{0}{0}{0}, terminal, el=S]
        ]
        [,p3,name=p3,el={$j=3$},tier=4
            [\util{0}{0}{\frac{1}{2}}, terminal, el=H]
            [\util{0}{0}{0}, terminal, el=S]
        ]
        [,nat,el={$j=\bot$}
        [,p1,name=p11,el={$k=1$} [\util{0}{0}{0}, terminal, el=H, draw]
        [,p2,name=p21,el=S [\util{0}{0}{0}, terminal, el=H]
        [,p3,name=p31,el=S,tier=4 [\util{0}{0}{0}, terminal, el=H]
            [\util{1}{1}{1}, terminal,el=S]]]]
        [,p2,name=p22,el={$k=2$} [\util{0}{0}{0}, terminal, el=H, draw]
        [,p3,name=p32,el=S [\util{0}{0}{0}, terminal, el=H]
        [,p1,name=p12,el=S,tier=4 [\util{0}{0}{0}, terminal, el=H]
            [\util{1}{1}{1}, terminal,el=S]]]]
        [,p3,name=p33,el={$k=3$}[\util{0}{0}{0}, terminal, el=H, draw]
        [,p1,name=p13,el=S [\util{0}{0}{0}, terminal, el=H]
        [,p2,name=p23,el=S,tier=4 [\util{0}{0}{0}, terminal, el=H]
            [\util{1}{1}{1}, terminal,el=S]]]]
        ]
        ]
        % \begin{scope}[on background layer]
        \draw[infoset1] (p1) to (p11);
        \draw[infoset1, bend right=15] (p11) to (p12);
        \draw[infoset1] (p12) to (p13);
        \draw[infoset2, bend right=15] (p2) to (p21);
        \draw[infoset2] (p21) to (p22);
        \draw[infoset2, bend right=15] (p22) to (p23);
        \draw[infoset3, bend right=30] (p3) to (p31);
        \draw[infoset3] (p31) to (p32) to (p33);
        % \end{scope}
    \end{forest}}%
% \label{fi:staghunt-body}


==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}

\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

==> tables/dag_sizes_nfcce_efcce_efce_comm.tex <==
\begin{tabular}{l|rr|rr|rr|rr} %%%% ['nfcce', 'efcce', 'efce', 'comm']
    \toprule
    \multirow{2}{*}{\bf Game}& \multicolumn{2}{c|}{NFCCE}& \multicolumn{2}{c|}{EFCCE}& \multicolumn{2}{c|}{EFCE}& \multicolumn{2}{c}{COMM}\\
 & \textbf{Dec. pts.} & \textbf{Edges} & \textbf{Dec. pts.} & \textbf{Edges} & \textbf{Dec. pts.} & \textbf{Edges} & \textbf{Dec. pts.} & \textbf{Edges}\\
    \midrule
        \texttt{B2222} & \num{1429} & \num{6915} & \num{5001} & \num{21868} & \num{4212} & \num{20534} & \num{16341} & \num{65577}\\
        \texttt{B2322} & \num{11707} & \num{89519} & \num{66181} & \num{340619} & \num{67219} & \num{503145} & \num{681523} & \num{4090261}\\
        \texttt{B2323} & \num{164707} & \num{1022286} & \num{1067881} & \num{5446015} & \num{1032019} & \num{7271972} & \unk & \unk\\
        \texttt{B2324} & \num{1316707} & \num{6397418} & \num{8296681} & \num{41633816} & \num{8160018} & \num{49264667} & \unk & \unk\\
    \midrule
        \texttt{D32} & \num{3956} & \num{33823} & \num{5381} & \num{51593} & \num{53402} & \num{536485} & \num{12794} & \num{45070}\\
        \texttt{D33} & \num{417625} & \num{11165451} & \num{1599919} & \num{71372690} & \unk & \unk & \num{2854524} & \num{10450812}\\
    \midrule
        \texttt{GL3} & \num{8898} & \num{30021} & \num{10680} & \num{37041} & \num{5637} & \num{16950} & \num{182289} & \num{547086}\\
    \midrule
        \texttt{K35} & \num{52277} & \num{3592121} & \num{60257} & \num{3826201} & \num{61217} & \num{4535281} & \num{9745} & \num{29235}\\
    \midrule
        \texttt{L3132} & \num{131012} & \num{1222128} & \num{689890} & \num{15329595} & \num{694381} & \num{8400513} & \num{326730} & \num{980190}\\
        \texttt{L3133} & \num{155297} & \num{1500087} & \num{1002685} & \num{26166405} & \num{1010749} & \num{14519676} & \num{365187} & \num{1095561}\\
        \texttt{L3151} & \num{1697120} & \num{34405970} & \unk & \unk & \unk & \unk & \num{1784965} & \num{5354895}\\
        \texttt{L3223} & \num{91735} & \num{614847} & \num{405691} & \num{5617510} & \num{678365} & \num{4999142} & \num{1234394} & \num{4004046}\\
        \texttt{L3523} & \num{7595335} & \num{58635336} & \unk & \unk & \unk & \unk & \unk & \unk\\
    \midrule
        \texttt{S2122} & \num{651} & \num{2903} & \num{2061} & \num{7847} & \num{1629} & \num{6227} & \num{4071} & \num{12629}\\
        \texttt{S2123} & \num{4413} & \num{19049} & \num{17883} & \num{72377} & \num{13113} & \num{52559} & \num{146631} & \num{454565}\\
        \texttt{S2133} & \num{9424} & \num{45931} & \num{40960} & \num{171915} & \num{38732} & \num{165859} & \num{778108} & \num{2425875}\\
        \texttt{S2254} & \num{617056} & \num{3758737} & \num{3974008} & \num{18655297} & \num{5470186} & \num{25303237} & \unk & \unk\\
        \texttt{S2264} & \num{1103369} & \num{7284509} & \num{7291859} & \num{34837769} & \unk & \unk & \unk & \unk\\
    \midrule
        \texttt{TP3} & \num{2355864} & \num{7145312} & \num{3574464} & \num{11720048} & \num{2211712} & \num{6714256} & \unk & \unk\\
    \midrule
        \texttt{U212} & \num{658} & \num{15410} & \num{658} & \num{10604} & \num{538} & \num{9000} & \num{3317} & \num{14338}\\
        \texttt{U213} & \num{61122} & \num{95194268} & \num{62704} & \num{95250604} & \num{97070} & \num{124453191} & \num{365621} & \num{1638786}\\
        \texttt{U222} & \num{1625} & \num{55123} & \num{1625} & \num{35047} & \num{1495} & \num{32643} & \num{4142} & \num{15914}\\
        \texttt{U223} & \unk & \unk & \unk & \unk & \unk & \unk & \num{299162} & \num{1184114}\\
    \bottomrule
\end{tabular}

==> tables/dag_sizes_nfccert_ccert_cert.tex <==
\begin{tabular}{l|rr|rr|rr} %%%% ['nfccert', 'ccert', 'cert']
    \toprule
    \multirow{2}{*}{\bf Game}& \multicolumn{2}{c|}{NFCCERT}& \multicolumn{2}{c|}{CCERT}& \multicolumn{2}{c|}{CERT}\\
 & \textbf{Dec. pts.} & \textbf{Edges} & \textbf{Dec. pts.} & \textbf{Edges} & \textbf{Dec. pts.} & \textbf{Edges}\\
    \midrule
        \texttt{B2222} & \num{663} & \num{2739} & \num{1430} & \num{5854} & \num{3590} & \num{14638}\\
        \texttt{B2322} & \num{5661} & \num{34227} & \num{13940} & \num{84080} & \num{52640} & \num{317180}\\
        \texttt{B2323} & \num{77661} & \num{394227} & \num{244340} & \num{1236080} & \num{959840} & \num{4853180}\\
        \texttt{B2324} & \num{596061} & \num{2467827} & \num{2188340} & \num{9012080} & \num{8476640} & \num{34920380}\\
    \midrule
        \texttt{D32} & \num{472} & \num{1796} & \num{504} & \num{1844} & \num{2484} & \num{9176}\\
        \texttt{D33} & \num{11292} & \num{44382} & \num{18396} & \num{68937} & \num{135504} & \num{520665}\\
    \midrule
        \texttt{GL3} & \num{2343} & \num{7104} & \num{3138} & \num{9474} & \num{5058} & \num{15234}\\
    \midrule
        \texttt{K35} & \num{1005} & \num{3015} & \num{1075} & \num{3225} & \num{2315} & \num{6945}\\
    \midrule
        \texttt{L3132} & \num{7773} & \num{23319} & \num{15789} & \num{47367} & \num{32055} & \num{96165}\\
        \texttt{L3133} & \num{9960} & \num{29880} & \num{21534} & \num{64602} & \num{44868} & \num{134604}\\
        \texttt{L3151} & \num{18285} & \num{54855} & \num{36115} & \num{108345} & \num{72395} & \num{217185}\\
        \texttt{L3223} & \num{14186} & \num{46656} & \num{36298} & \num{118576} & \num{83786} & \num{273276}\\
        \texttt{L3523} & \num{1115978} & \num{3887736} & \num{5617402} & \num{19357364} & \num{14863826} & \num{51214448}\\
    \midrule
        \texttt{S2122} & \num{408} & \num{1396} & \num{825} & \num{2627} & \num{1749} & \num{5465}\\
        \texttt{S2123} & \num{2496} & \num{8452} & \num{6873} & \num{21959} & \num{15717} & \num{49349}\\
        \texttt{S2133} & \num{5112} & \num{18566} & \num{15000} & \num{49607} & \num{44084} & \num{139851}\\
        \texttt{S2254} & \num{327992} & \num{1300694} & \num{1332064} & \num{4615207} & \num{6089698} & \num{19348765}\\
        \texttt{S2264} & \num{579182} & \num{2358134} & \num{2402695} & \num{8425369} & \num{12809119} & \num{40551631}\\
    \midrule
        \texttt{TP3} & \num{1070544} & \num{3273072} & \num{1739488} & \num{5273184} & \num{3594352} & \num{10896416}\\
    \midrule
        \texttt{U212} & \num{213} & \num{902} & \num{182} & \num{768} & \num{182} & \num{768}\\
        \texttt{U213} & \num{2459} & \num{10870} & \num{2808} & \num{12416} & \num{4288} & \num{19160}\\
        \texttt{U222} & \num{290} & \num{1098} & \num{252} & \num{952} & \num{252} & \num{952}\\
        \texttt{U223} & \num{2778} & \num{10854} & \num{3224} & \num{12600} & \num{4500} & \num{17776}\\
    \bottomrule
\end{tabular}

==> tables/detailed/comparison_ccert_2pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize social welfare}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
\midrule \texttt{B2222} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] \\
         \texttt{B2322} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.07s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.22s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.15s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.34s} & [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.22s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.33s} &  [1.0] \\
         \texttt{B2323} & \cbox{0.8692041522491349,0.8692041522491349,0.9681660899653979}{7.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.75s} &  [1.0] &    \cbox{0.875355632449058,0.875355632449058,0.9658592848904267}{7.37s} &  [1.0] & \cbox{0.8175317185697808,0.8175317185697808,0.9875432525951557}{6.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{4.69s} &  [1.0] & \cbox{0.8839677047289504,0.8839677047289504,0.9626297577854671}{9.79s} & [1.0] &  \cbox{0.8372164552095348,0.8372164552095348,0.980161476355248}{8.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{5.39s} &  [1.0] &   \cbox{0.8003075740099962,0.8003075740099962,0.994002306805075}{6.08s} &  [1.0] \\
         \texttt{B2324} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{54.92s} &  [1.0] &  \cbox{0.8027681660899654,0.8027681660899654,0.9930795847750865}{1m 2s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{59.02s} &  [1.0] &  \cbox{0.839677047289504,0.839677047289504,0.9792387543252595}{1m 28s} & [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 31s} &  [1.0] & \cbox{0.7978469819300269,0.7978469819300269,0.9949250288350634}{1m 41s} &  [1.0] \\
\midrule \texttt{S2122} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] \\
         \texttt{S2123} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} & [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [1.0] \\
         \texttt{S2133} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.07s} &  [1.0] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.08s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.09s} & [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.11s} &  [1.0] \\
         \texttt{S2254} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{1m 41s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{8.61s} &  [0.1] &  \cbox{0.8630526720492118,0.8630526720492118,0.970472895040369}{15.31s} &  [0.1] & \cbox{0.960322952710496,0.8901191849288735,0.8901191849288735}{1m 47s} & \cbox{0.7953863898500576,0.7953863898500576,0.995847750865052}{25.38s} &  [0.1] &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{23.28s} & [0.1] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{2m 3s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{8.22s} &  [0.1] &   \cbox{0.875355632449058,0.875355632449058,0.9658592848904267}{16.08s} &  [0.1] \\
         \texttt{S2264} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{20.11s} &  [1.0] & \cbox{0.8076893502499038,0.8076893502499038,0.9912341407151096}{23.99s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7929257977700884,0.7929257977700884,0.9967704728950404}{1m 9s} & [0.01] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 5s} & [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{16.50s} &  [0.1] & \cbox{0.8605920799692426,0.8605920799692426,0.9713956170703576}{29.02s} &  [0.1] \\
 \midrule \texttt{RS212} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] \\
          \texttt{RS222} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] \\
          \texttt{RS213} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [0.01] \\
          \texttt{RS223} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_ccert_3pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize Player~3's utility}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
  \midrule \texttt{D32} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] \\
           \texttt{D33} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.20s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.29s} &  [1.0] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.13s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.30s} &  [1.0] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.31s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.19s} &  [0.1] \\
  \midrule \texttt{GL3} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] \\
  \midrule \texttt{K35} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] \\
\midrule \texttt{L3132} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.06s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.07s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.06s} &  [0.1] \\
         \texttt{L3133} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.08s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.11s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.12s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.15s} &  [0.1] \\
         \texttt{L3151} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.12s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.27s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.16s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.35s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.16s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.33s} &  [0.1] \\
         \texttt{L3223} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.23s} &  [0.1] &      \cbox{0.78800461361015,0.78800461361015,0.9986159169550173}{0.52s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.26s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.43s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.24s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.41s} & [0.01] \\
         \texttt{L3523} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 17s} & [0.01] &  \cbox{0.8901191849288735,0.8901191849288735,0.960322952710496}{2m 47s} & [0.01] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 16s} & [0.01] &  \cbox{0.9061130334486736,0.9061130334486736,0.9543252595155709}{3m 6s} & [0.01] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 13s} & [0.01] & \cbox{0.8778162245290273,0.8778162245290273,0.9649365628604383}{2m 26s} & [0.01] \\
  \midrule \texttt{TP3} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{10.23s} & [10.0] & \cbox{0.8605920799692426,0.8605920799692426,0.9713956170703576}{18.00s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{10.38s} & [10.0] & \cbox{0.8728950403690888,0.8728950403690888,0.9667820069204152}{19.88s} & [10.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{11.95s} & [10.0] & \cbox{0.8888888888888888,0.8888888888888888,0.9607843137254902}{25.89s} & [10.0] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_cert_2pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize social welfare}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
\midrule \texttt{B2222} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] \\
         \texttt{B2322} & \cbox{0.8716647443291041,0.8716647443291041,0.9672433679354094}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.05s} &  [1.0] &  \cbox{0.7966166858900423,0.7966166858900423,0.9953863898500577}{1.16s} &  [1.0] &  \cbox{0.8581314878892734,0.8581314878892734,0.972318339100346}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.16s} &  [1.0] &  \cbox{0.8765859284890427,0.8765859284890427,0.9653979238754326}{2.29s} &  [1.0] &   \cbox{0.849519415609381,0.849519415609381,0.9755478662053056}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.24s} &  [1.0] &     \cbox{0.80399846212995,0.80399846212995,0.9926182237600922}{1.43s} &  [1.0] \\
         \texttt{B2323} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{40.00s} & \cbox{0.8064590542099193,0.8064590542099193,0.9916955017301038}{47.11s} & [10.0] &  \cbox{0.8445982314494425,0.8445982314494425,0.9773933102652825}{1m 2s} &  [1.0] &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{33.00s} & \cbox{0.8618223760092272,0.8618223760092272,0.9709342560553633}{58.20s} &  [1.0] & \cbox{0.9543252595155709,0.9061130334486736,0.9061130334486736}{2m 14s} &  [0.1] &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{37.00s} & \cbox{0.8150711264898116,0.8150711264898116,0.9884659746251442}{46.51s} &  [1.0] & \cbox{0.7953863898500576,0.7953863898500576,0.995847750865052}{40.45s} &  [1.0] \\
         \texttt{B2324} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{8m 29s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{6m 14s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & [\unk] \\
\midrule \texttt{S2122} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] \\
         \texttt{S2123} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.19s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.37s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.28s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.31s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.15s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.35s} &  [0.1] \\
         \texttt{S2133} & \cbox{0.9393310265282584,0.9393310265282584,0.9418685121107266}{3.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.96s} &  [1.0] &  \cbox{0.7966166858900423,0.7966166858900423,0.9953863898500577}{1.06s} &  [1.0] & \cbox{0.8655132641291811,0.8655132641291811,0.9695501730103806}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.10s} &  [0.1] &    \cbox{0.794156093810073,0.794156093810073,0.9963091118800461}{1.18s} &  [0.1] &  \cbox{0.8901191849288735,0.8901191849288735,0.960322952710496}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.92s} &  [0.1] & \cbox{0.8273740868896579,0.8273740868896579,0.9838523644752019}{1.26s} &  [0.1] \\
         \texttt{S2254} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3m 26s} &  [0.1] & \cbox{0.8507497116493656,0.8507497116493656,0.9750865051903114}{5m 35s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7867743175701654,0.7867743175701654,0.9990772779700116}{6m 23s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{6m 15s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{2m 42s} &  [0.1] & \cbox{0.9319492502883506,0.9319492502883506,0.9446366782006921}{8m 2s} &  [0.1] \\
         \texttt{S2264} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
 \midrule \texttt{RS212} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] \\
          \texttt{RS222} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] \\
          \texttt{RS213} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} & [10.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] \\
          \texttt{RS223} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} & [0.01] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_cert_3pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize Player~3's utility}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
  \midrule \texttt{D32} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] \\
           \texttt{D33} & \cbox{0.8163014225297962,0.8163014225297962,0.9880046136101499}{4.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.14s} &  [1.0] &   \cbox{0.8741253364090734,0.8741253364090734,0.966320645905421}{6.08s} &  [1.0] & \cbox{0.8778162245290273,0.8778162245290273,0.9649365628604383}{4.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{2.02s} &  [1.0] &  \cbox{0.8458285274894272,0.8458285274894272,0.9769319492502884}{3.18s} &  [0.1] & \cbox{0.8716647443291041,0.8716647443291041,0.9672433679354094}{4.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{2.10s} &  [1.0] & \cbox{0.8679738562091504,0.8679738562091504,0.9686274509803922}{3.89s} &  [0.1] \\
  \midrule \texttt{GL3} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] \\
  \midrule \texttt{K35} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] \\
\midrule \texttt{L3132} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.15s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.10s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.18s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.22s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.18s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.35s} &  [0.1] \\
         \texttt{L3133} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.22s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.42s} &  [1.0] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.19s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.33s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.25s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.38s} &  [0.1] \\
         \texttt{L3151} & \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.21s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.42s} &  [0.1] & \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.22s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.44s} &  [0.1] & \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.29s} &  [0.1] & \cbox{0.7916955017301038,0.7916955017301038,0.9972318339100346}{0.53s} &  [0.1] \\
         \texttt{L3223} & \cbox{0.8507497116493656,0.8507497116493656,0.9750865051903114}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.61s} &  [0.1] &  \cbox{0.8999615532487505,0.8999615532487505,0.9566320645905421}{1.43s} & [0.01] & \cbox{0.8519800076893502,0.8519800076893502,0.9746251441753172}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.61s} &  [0.1] &  \cbox{0.8679738562091504,0.8679738562091504,0.9686274509803922}{1.13s} & [0.01] & \cbox{0.8359861591695501,0.8359861591695501,0.9806228373702423}{1.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.68s} &  [0.1] & \cbox{0.8335255670895809,0.8335255670895809,0.9815455594002307}{0.98s} & [0.01] \\
         \texttt{L3523} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{2m 58s} & [0.01] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & [\unk] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{4m 33s} & [0.01] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & [\unk] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{3m 55s} & [0.01] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & [\unk] \\
  \midrule \texttt{TP3} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{26.70s} &  [1.0] & \cbox{0.8409073433294887,0.8409073433294887,0.9787773933102653}{40.73s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{25.08s} &  [1.0] & \cbox{0.8335255670895809,0.8335255670895809,0.9815455594002307}{35.99s} & [10.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{36.36s} & [10.0] & \cbox{0.8519800076893502,0.8519800076893502,0.9746251441753172}{1m 0s} &  [1.0] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_comm_2pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize social welfare}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
\midrule \texttt{B2222} &  \cbox{0.8962706651287966,0.8962706651287966,0.9580161476355248}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.88s} &  [1.0] &   \cbox{0.8187620146097655,0.8187620146097655,0.9870818915801615}{1.14s} &  [1.0] & \cbox{0.8938100730488273,0.8938100730488273,0.9589388696655132}{2.00s} &  \cbox{0.8273740868896579,0.8273740868896579,0.9838523644752019}{1.23s} & [10.0] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.89s} &  [1.0] &    \cbox{0.823683198769704,0.823683198769704,0.9852364475201846}{2.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.49s} & [10.0] &   \cbox{0.8445982314494425,0.8445982314494425,0.9773933102652825}{2.33s} &  [1.0] \\
         \texttt{B2322} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{5m 47s} &  [1.0] & \cbox{0.8618223760092272,0.8618223760092272,0.9709342560553633}{10m 17s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3m 45s} &  [1.0] &     \cbox{0.823683198769704,0.823683198769704,0.9852364475201846}{5m 2s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{4m 41s} &  [1.0] &   \cbox{0.8409073433294887,0.8409073433294887,0.9787773933102653}{7m 6s} &  [1.0] \\
         \texttt{B2323} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
         \texttt{B2324} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
\midrule \texttt{S2122} &  \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.21s} &  [0.1] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.36s} &  [0.1] & \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.48s} & [0.01] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.48s} &  [0.1] &  \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.36s} & [0.01] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.35s} &  [0.1] \\
         \texttt{S2123} & \cbox{0.8987312572087658,0.8987312572087658,0.9570934256055363}{1m 30s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{38.95s} &  [0.1] &     \cbox{0.859361783929258,0.859361783929258,0.9718569780853518}{1m 7s} &  [0.1] & \cbox{0.8261437908496732,0.8261437908496732,0.984313725490196}{1m 36s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 10s} & [0.01] &  \cbox{0.8482891195693963,0.8482891195693963,0.9760092272202999}{1m 52s} & [0.01] & \cbox{0.8445982314494425,0.8445982314494425,0.9773933102652825}{1m 33s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{59.63s} & [0.01] &  \cbox{0.8409073433294887,0.8409073433294887,0.9787773933102653}{1m 30s} &  [0.1] \\
         \texttt{S2133} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.8569011918492887,0.8569011918492887,0.9727797001153402}{7m 34s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{4m 26s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{7m 27s} & [0.01] & \cbox{0.8716647443291041,0.8716647443291041,0.9672433679354094}{14m 12s} & [0.01] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &              \cbox{0.7843137254901961,0.7843137254901961,1.0}{12m 11s} & [0.01] & \cbox{0.7990772779700115,0.7990772779700115,0.9944636678200692}{13m 40s} & [0.01] \\
         \texttt{S2254} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
         \texttt{S2264} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &   \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
 \midrule \texttt{RS212} &  \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] & \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} & [10.0] &  \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] \\
          \texttt{RS222} &  \cbox{0.9741637831603229,0.8532103037293348,0.8532103037293348}{3.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] & \cbox{0.9741637831603229,0.8532103037293348,0.8532103037293348}{3.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} & [10.0] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [1.0] &  \cbox{0.9741637831603229,0.8532103037293348,0.8532103037293348}{3.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} & [10.0] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [0.01] \\
          \texttt{RS213} &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{6m 51s} &   \cbox{0.794156093810073,0.794156093810073,0.9963091118800461}{11.05s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{10.24s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{6m 27s} & \cbox{0.8015378700499808,0.8015378700499808,0.9935409457900808}{14.66s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{12.83s} &  [1.0] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{6m 25s} &     \cbox{0.78800461361015,0.78800461361015,0.9986159169550173}{9.00s} &  [1.0] &                  \cbox{0.7843137254901961,0.7843137254901961,1.0}{8.74s} &  [1.0] \\
          \texttt{RS223} &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{8m 41s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{5.79s} & [10.0] &  \cbox{0.8655132641291811,0.8655132641291811,0.9695501730103806}{10.49s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{8m 24s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{8.45s} &  [1.0] &   \cbox{0.8212226066897347,0.8212226066897347,0.986159169550173}{11.14s} &  [1.0] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{8m 54s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{4.00s} &  [1.0] &   \cbox{0.8605920799692426,0.8605920799692426,0.9713956170703576}{7.02s} &  [1.0] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_comm_3pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize Player~3's utility}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
  \midrule \texttt{D32} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.06s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.12s} &  [1.0] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.06s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.18s} &  [0.1] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.18s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.17s} &  [1.0] \\
           \texttt{D33} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{4m 37s} &  [1.0] & \cbox{0.8864282968089197,0.8864282968089197,0.9617070357554787}{9m 46s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 31s} &  [1.0] &  \cbox{0.8802768166089965,0.8802768166089965,0.9640138408304498}{3m 5s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{2m 38s} &  [1.0] & \cbox{0.8384467512495194,0.8384467512495194,0.9797001153402537}{3m 57s} &  [0.1] \\
  \midrule \texttt{GL3} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{7.72s} &  [0.1] & \cbox{0.8347558631295655,0.8347558631295655,0.9810841983852364}{11.24s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{7.50s} &  [1.0] & \cbox{0.8359861591695501,0.8359861591695501,0.9806228373702423}{11.02s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{11.42s} &  [1.0] & \cbox{0.8470588235294118,0.8470588235294118,0.9764705882352941}{18.22s} &  [0.1] \\
  \midrule \texttt{K35} &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [1.0] \\
\midrule \texttt{L3132} &  \cbox{0.8987312572087658,0.8987312572087658,0.9570934256055363}{8.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.46s} &  [0.1] &  \cbox{0.8507497116493656,0.8507497116493656,0.9750865051903114}{5.65s} &  [0.1] &  \cbox{0.9024221453287197,0.9024221453287197,0.9557093425605536}{8.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.37s} &  [0.1] &  \cbox{0.8605920799692426,0.8605920799692426,0.9713956170703576}{5.89s} &  [0.1] &    \cbox{0.859361783929258,0.859361783929258,0.9718569780853518}{7.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{4.02s} &  [0.1] &  \cbox{0.8839677047289504,0.8839677047289504,0.9626297577854671}{8.38s} &  [0.1] \\
         \texttt{L3133} & \cbox{0.9469434832756632,0.9257977700884276,0.9257977700884276}{12.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.40s} &  [0.1] &  \cbox{0.8999615532487505,0.8999615532487505,0.9566320645905421}{7.98s} &  [0.1] & \cbox{0.9446366782006921,0.9319492502883506,0.9319492502883506}{12.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.54s} &  [0.1] &  \cbox{0.8925797770088427,0.8925797770088427,0.9594002306805075}{7.89s} &  [0.1] & \cbox{0.9393310265282584,0.9393310265282584,0.9418685121107266}{11.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.52s} &  [0.1] & \cbox{0.9331795463283352,0.9331795463283352,0.9441753171856978}{10.52s} &  [0.1] \\
         \texttt{L3151} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{16.73s} &  [0.1] & \cbox{0.7966166858900423,0.7966166858900423,0.9953863898500577}{18.42s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{15.80s} &  [0.1] & \cbox{0.8692041522491349,0.8692041522491349,0.9681660899653979}{29.51s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{18.00s} &  [0.1] &   \cbox{0.813840830449827,0.813840830449827,0.9889273356401385}{22.54s} &  [0.1] \\
         \texttt{L3223} & \cbox{0.7892349096501345,0.7892349096501345,0.9981545559400231}{19.00s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{18.19s} &  [0.1] & \cbox{0.8482891195693963,0.8482891195693963,0.9760092272202999}{29.24s} & [0.01] & \cbox{0.8064590542099193,0.8064590542099193,0.9916955017301038}{18.00s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{15.30s} &  [0.1] &  \cbox{0.8630526720492118,0.8630526720492118,0.970472895040369}{27.38s} &  [0.1] & \cbox{0.7990772779700115,0.7990772779700115,0.9944636678200692}{21.00s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{18.77s} &  [0.1] & \cbox{0.8273740868896579,0.8273740868896579,0.9838523644752019}{25.91s} & [0.01] \\
         \texttt{L3523} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
  \midrule \texttt{TP3} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_efcce_2pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize social welfare}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
\midrule \texttt{B2222} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] \\
         \texttt{B2322} & \cbox{0.9741637831603229,0.8532103037293348,0.8532103037293348}{3.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.41s} &  [1.0] &    \cbox{0.895040369088812,0.895040369088812,0.9584775086505191}{1.13s} &  [1.0] &  \cbox{0.9575547866205305,0.8975009611687812,0.8975009611687812}{3.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.69s} &  [1.0] &  \cbox{0.8569011918492887,0.8569011918492887,0.9727797001153402}{1.19s} &  [1.0] &  \cbox{0.9570934256055363,0.8987312572087659,0.8987312572087659}{3.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.69s} &  [1.0] &  \cbox{0.8728950403690888,0.8728950403690888,0.9667820069204152}{1.33s} &  [1.0] \\
         \texttt{B2323} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{1m 35s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{9.11s} &  [1.0] & \cbox{0.9061130334486736,0.9061130334486736,0.9543252595155709}{22.38s} &  [1.0] & \cbox{0.9838523644752019,0.8273740868896579,0.8273740868896579}{1m 30s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{12.39s} &  [1.0] & \cbox{0.8716647443291041,0.8716647443291041,0.9672433679354094}{23.59s} &  [1.0] & \cbox{0.9713956170703576,0.8605920799692426,0.8605920799692426}{1m 21s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{14.23s} &  [1.0] & \cbox{0.8322952710495963,0.8322952710495963,0.9820069204152249}{20.30s} &  [1.0] \\
         \texttt{B2324} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 53s} &  [1.0] & \cbox{0.8716647443291041,0.8716647443291041,0.9672433679354094}{3m 35s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{2m 44s} &  [1.0] & \cbox{0.8519800076893502,0.8519800076893502,0.9746251441753172}{4m 29s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3m 1s} &  [1.0] & \cbox{0.8310649750096116,0.8310649750096116,0.9824682814302191}{4m 16s} &  [1.0] \\
\midrule \texttt{S2122} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] \\
         \texttt{S2123} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.19s} &  [0.1] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.09s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [0.1] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.06s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.16s} &  [1.0] \\
         \texttt{S2133} & \cbox{0.9741637831603229,0.8532103037293348,0.8532103037293348}{3.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.12s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.31s} &  [1.0] &  \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.20s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.22s} &  [0.1] &  \cbox{0.9741637831603229,0.8532103037293348,0.8532103037293348}{3.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.11s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.41s} &  [1.0] \\
         \texttt{S2254} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7904652056901191,0.7904652056901191,0.9976931949250288}{28.81s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{27.31s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{37.43s} &  [0.1] & \cbox{0.8310649750096116,0.8310649750096116,0.9824682814302191}{53.08s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{22.01s} &  [1.0] & \cbox{0.8544405997693195,0.8544405997693195,0.9737024221453288}{36.83s} &  [0.1] \\
         \texttt{S2264} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{46.07s} &  [0.1] & \cbox{0.8667435601691656,0.8667435601691656,0.9690888119953864}{1m 24s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{2m 18s} &  [0.1] & \cbox{0.7904652056901191,0.7904652056901191,0.9976931949250288}{2m 26s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{39.23s} &  [0.1] &  \cbox{0.8618223760092272,0.8618223760092272,0.9709342560553633}{1m 9s} &  [0.1] \\
 \midrule \texttt{RS212} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] \\
          \texttt{RS222} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] \\
          \texttt{RS213} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{28.80s} &  [1.0] & \cbox{0.9510957324106113,0.9147251057285659,0.9147251057285659}{1m 50s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{31.02s} &  [1.0] & \cbox{0.8987312572087658,0.8987312572087658,0.9570934256055363}{1m 11s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{15.54s} &  [0.1] &   \cbox{0.904882737408689,0.904882737408689,0.9547866205305652}{37.73s} &  [0.1] \\
          \texttt{RS223} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_efcce_3pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize Player~3's utility}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
  \midrule \texttt{D32} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] \\
           \texttt{D33} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 46s} &  [1.0] &    \cbox{0.911034217608612,0.911034217608612,0.952479815455594}{4m 31s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 16s} &  [1.0] & \cbox{0.9368704344482891,0.9368704344482891,0.9427912341407151}{3m 56s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 44s} &  [1.0] &  \cbox{0.9270280661284122,0.9270280661284122,0.946482122260669}{4m 56s} &  [1.0] \\
  \midrule \texttt{GL3} & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [1.0] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [1.0] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} & [10.0] \\
  \midrule \texttt{K35} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{46.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.67s} & [10.0] &     \cbox{0.911034217608612,0.911034217608612,0.952479815455594}{1.69s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{55.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.75s} &  [1.0] &    \cbox{0.895040369088812,0.895040369088812,0.9584775086505191}{1.69s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{51.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.68s} &  [1.0] &  \cbox{0.9319492502883506,0.9319492502883506,0.9446366782006921}{2.02s} &  [0.1] \\
\midrule \texttt{L3132} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{8m 43s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{5.13s} &  [0.1] &  \cbox{0.8692041522491349,0.8692041522491349,0.9681660899653979}{9.57s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{9m 17s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{6.27s} &  [0.1] & \cbox{0.8765859284890427,0.8765859284890427,0.9653979238754326}{12.37s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{9m 44s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{7.76s} &  [0.1] & \cbox{0.8704344482891195,0.8704344482891195,0.9677047289504037}{14.66s} &  [0.1] \\
         \texttt{L3133} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{20m 26s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{8.88s} &  [0.1] & \cbox{0.8827374086889658,0.8827374086889658,0.9630911188004614}{18.30s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{8.19s} &  [1.0] & \cbox{0.8925797770088427,0.8925797770088427,0.9594002306805075}{18.09s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{23m 15s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{10.86s} &  [1.0] & \cbox{0.8569011918492887,0.8569011918492887,0.9727797001153402}{18.52s} &  [0.1] \\
         \texttt{L3151} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
         \texttt{L3223} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{1m 10s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{2.94s} &  [0.1] &  \cbox{0.8519800076893502,0.8519800076893502,0.9746251441753172}{4.85s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{1m 10s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.22s} &  [0.1] &  \cbox{0.8359861591695501,0.8359861591695501,0.9806228373702423}{4.73s} &  [0.1] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{1m 2s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.24s} &  [0.1] &   \cbox{0.8372164552095348,0.8372164552095348,0.980161476355248}{4.78s} &  [0.1] \\
         \texttt{L3523} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
  \midrule \texttt{TP3} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{13.76s} & [10.0] & \cbox{0.8655132641291811,0.8655132641291811,0.9695501730103806}{24.94s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{15.03s} & [10.0] & \cbox{0.8704344482891195,0.8704344482891195,0.9677047289504037}{28.28s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{15.27s} & [10.0] &  \cbox{0.8630526720492118,0.8630526720492118,0.970472895040369}{27.29s} &  [1.0] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_efce_2pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize social welfare}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
\midrule \texttt{B2222} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.06s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] \\
         \texttt{B2322} &   \cbox{0.984313725490196,0.8261437908496732,0.8261437908496732}{9.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.23s} &  [1.0] &  \cbox{0.9036524413687044,0.9036524413687044,0.9552479815455593}{2.97s} &  [1.0] &  \cbox{0.8741253364090734,0.8741253364090734,0.966320645905421}{9.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{4.63s} &  [1.0] &  \cbox{0.7855440215301807,0.7855440215301807,0.9995386389850057}{4.68s} &  [1.0] &   \cbox{0.970472895040369,0.8630526720492118,0.8630526720492118}{9.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.60s} & [10.0] &  \cbox{0.8642829680891965,0.8642829680891965,0.9700115340253749}{2.88s} &  [1.0] \\
         \texttt{B2323} & \cbox{0.9630911188004614,0.8827374086889658,0.8827374086889658}{3m 54s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{48.40s} &  [1.0] & \cbox{0.8655132641291811,0.8655132641291811,0.9695501730103806}{1m 28s} &  [1.0] &  \cbox{0.9270280661284122,0.9270280661284122,0.946482122260669}{4m 9s} & \cbox{0.7990772779700115,0.7990772779700115,0.9944636678200692}{1m 38s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 27s} &  [1.0] & \cbox{0.9635524798154556,0.8815071126489812,0.8815071126489812}{3m 40s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{45.12s} & [10.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{44.87s} &  [1.0] \\
         \texttt{B2324} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{9m 3s} &  [1.0] & \cbox{0.8347558631295655,0.8347558631295655,0.9810841983852364}{13m 8s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & [\unk] &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{10m 21s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.823683198769704,0.823683198769704,0.9852364475201846}{14m 30s} &  [1.0] &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{10m 48s} &  [1.0] \\
\midrule \texttt{S2122} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] \\
         \texttt{S2123} &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.09s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.23s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.34s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.43s} &  [1.0] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.15s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.25s} &  [0.1] \\
         \texttt{S2133} &  \cbox{0.9866205305651672,0.8199923106497501,0.8199923106497501}{4.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.52s} &  [1.0] &  \cbox{0.8359861591695501,0.8359861591695501,0.9806228373702423}{0.77s} &  [0.1] & \cbox{0.8962706651287966,0.8962706651287966,0.9580161476355248}{3.00s} &  \cbox{0.8310649750096116,0.8310649750096116,0.9824682814302191}{1.86s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.31s} &  [0.1] &  \cbox{0.9741637831603229,0.8532103037293348,0.8532103037293348}{3.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.49s} &  [1.0] &  \cbox{0.8728950403690888,0.8728950403690888,0.9667820069204152}{0.96s} &  [1.0] \\
         \texttt{S2254} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7904652056901191,0.7904652056901191,0.9976931949250288}{2m 17s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{2m 10s} &  [0.1] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{3m 34s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & [\unk] \\
         \texttt{S2264} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
 \midrule \texttt{RS212} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] \\
          \texttt{RS222} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] \\
          \texttt{RS213} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{35.37s} &  [1.0] & \cbox{0.9085736255286428,0.9085736255286428,0.9534025374855825}{1m 28s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{32.49s} &  [1.0] & \cbox{0.9196462898885044,0.9196462898885044,0.9492502883506344}{1m 27s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{23.37s} & [0.01] & \cbox{0.9073433294886581,0.9073433294886581,0.9538638985005767}{57.68s} & [0.01] \\
          \texttt{RS223} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_efce_3pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize Player~3's utility}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
  \midrule \texttt{D32} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{12.00s} & \cbox{0.8421376393694733,0.8421376393694733,0.9783160322952711}{0.76s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.40s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{11.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.35s} &  [1.0] &  \cbox{0.8556708958093041,0.8556708958093041,0.9732410611303345}{0.85s} &  [1.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{10.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.66s} &  [1.0] &  \cbox{0.8101499423298731,0.8101499423298731,0.9903114186851211}{0.80s} &  [1.0] \\
           \texttt{D33} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
  \midrule \texttt{GL3} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] \\
  \midrule \texttt{K35} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{57.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.55s} &  [1.0] &  \cbox{0.8765859284890427,0.8765859284890427,0.9653979238754326}{1.08s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{55.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.03s} &  [1.0] &  \cbox{0.8322952710495963,0.8322952710495963,0.9820069204152249}{1.47s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{60.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.26s} &  [1.0] &    \cbox{0.829834678969627,0.829834678969627,0.9829296424452134}{1.77s} &  [0.1] \\
\midrule \texttt{L3132} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{8m 18s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{6.10s} &  [0.1] &  \cbox{0.8187620146097655,0.8187620146097655,0.9870818915801615}{7.85s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{8m 57s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{7.65s} &  [0.1] & \cbox{0.8458285274894272,0.8458285274894272,0.9769319492502884}{12.08s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{7m 35s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{6.78s} &  [0.1] & \cbox{0.8716647443291041,0.8716647443291041,0.9672433679354094}{12.88s} &  [0.1] \\
         \texttt{L3133} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{21m 25s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{6.84s} &  [0.1] & \cbox{0.8716647443291041,0.8716647443291041,0.9672433679354094}{12.97s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{21m 43s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{10.76s} &  [0.1] & \cbox{0.8569011918492887,0.8569011918492887,0.9727797001153402}{18.44s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{19m 58s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{10.28s} &  [0.1] & \cbox{0.8409073433294887,0.8409073433294887,0.9787773933102653}{15.69s} &  [0.1] \\
         \texttt{L3151} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
         \texttt{L3223} &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{2m 2s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{5.52s} &  [0.1] &  \cbox{0.8470588235294118,0.8470588235294118,0.9764705882352941}{8.74s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{1m 50s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{6.46s} &  [0.1] & \cbox{0.8532103037293348,0.8532103037293348,0.9741637831603229}{10.70s} &  [0.1] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{2m 0s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{5.94s} &  [0.1] &  \cbox{0.8630526720492118,0.8630526720492118,0.970472895040369}{10.65s} &  [0.1] \\
         \texttt{L3523} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
  \midrule \texttt{TP3} &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{13.46s} & [10.0] &   \cbox{0.839677047289504,0.839677047289504,0.9792387543252595}{20.25s} &  [1.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{14.25s} &  [1.0] & \cbox{0.8445982314494425,0.8445982314494425,0.9773933102652825}{22.19s} & [10.0] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{14.48s} & [10.0] & \cbox{0.8359861591695501,0.8359861591695501,0.9806228373702423}{21.28s} &  [1.0] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_nfcce_2pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize social welfare}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
\midrule \texttt{B2222} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] \\
         \texttt{B2322} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.07s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [10.0] \\
         \texttt{B2323} &  \cbox{0.9797001153402537,0.8384467512495194,0.8384467512495194}{7.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.05s} &  [0.1] &  \cbox{0.8421376393694733,0.8421376393694733,0.9783160322952711}{1.61s} &  [0.1] &  \cbox{0.9737024221453288,0.8544405997693195,0.8544405997693195}{6.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.01s} &  [0.1] &    \cbox{0.849519415609381,0.849519415609381,0.9755478662053056}{1.63s} &  [0.1] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{6.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.33s} &  [0.1] &  \cbox{0.7904652056901191,0.7904652056901191,0.9976931949250288}{0.53s} & [10.0] \\
         \texttt{B2324} & \cbox{0.9418685121107266,0.9393310265282584,0.9393310265282584}{50.00s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{15.57s} &  [0.1] & \cbox{0.8175317185697808,0.8175317185697808,0.9875432525951557}{20.01s} &  [0.1] & \cbox{0.9282583621683967,0.9282583621683967,0.9460207612456747}{37.00s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{12.80s} &  [0.1] & \cbox{0.8507497116493656,0.8507497116493656,0.9750865051903114}{20.91s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{38.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{2.73s} &  [0.1] &  \cbox{0.8544405997693195,0.8544405997693195,0.9737024221453288}{4.57s} &  [1.0] \\
\midrule \texttt{S2122} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] \\
         \texttt{S2123} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] \\
         \texttt{S2133} &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] & \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] \\
         \texttt{S2254} &                 \cbox{1.0,0.7843137254901961,0.7843137254901961}{2m 1s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{6.96s} &  [0.1] & \cbox{0.8519800076893502,0.8519800076893502,0.9746251441753172}{11.43s} &  [0.1] & \cbox{0.9824682814302191,0.8310649750096117,0.8310649750096117}{1m 14s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{10.43s} &  [0.1] & \cbox{0.8556708958093041,0.8556708958093041,0.9732410611303345}{17.72s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{1m 58s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{7.43s} &  [0.1] & \cbox{0.8482891195693963,0.8482891195693963,0.9760092272202999}{11.88s} &  [0.1] \\
         \texttt{S2264} &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{3m 36s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{13.96s} &  [0.1] & \cbox{0.8532103037293348,0.8532103037293348,0.9741637831603229}{23.25s} &  [0.1] & \cbox{0.9875432525951557,0.8175317185697809,0.8175317185697809}{2m 24s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{18.46s} &  [0.1] & \cbox{0.8716647443291041,0.8716647443291041,0.9672433679354094}{35.04s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{3m 43s} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{11.74s} &  [0.1] & \cbox{0.8409073433294887,0.8409073433294887,0.9787773933102653}{17.91s} &  [0.1] \\
 \midrule \texttt{RS212} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] \\
          \texttt{RS222} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [0.01] \\
          \texttt{RS213} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{34.52s} &  [1.0] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1m 9s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{20.29s} &  [1.0] & \cbox{0.8815071126489812,0.8815071126489812,0.9635524798154556}{41.66s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &               \cbox{0.7843137254901961,0.7843137254901961,1.0}{14.68s} &  [0.1] & \cbox{0.9036524413687044,0.9036524413687044,0.9552479815455593}{35.36s} &  [0.1] \\
          \texttt{RS223} &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] &  \cbox{0.9414071510957324,0.940561322568243,0.940561322568243}{timeout} & [\unk] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_nfcce_3pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize Player~3's utility}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
  \midrule \texttt{D32} &              \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] \\
           \texttt{D33} &             \cbox{1.0,0.7843137254901961,0.7843137254901961}{2m 17s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{12.93s} &  [0.1] & \cbox{0.9441753171856978,0.9331795463283352,0.9331795463283352}{43.45s} &  [0.1] & \cbox{0.9875432525951557,0.8175317185697809,0.8175317185697809}{2m 8s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{16.40s} &  [0.1] & \cbox{0.8815071126489812,0.8815071126489812,0.9635524798154556}{33.57s} &  [0.1] & \cbox{0.9898500576701269,0.8113802383698577,0.8113802383698577}{2m 23s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{17.57s} &  [0.1] & \cbox{0.8839677047289504,0.8839677047289504,0.9626297577854671}{36.55s} &  [1.0] \\
  \midrule \texttt{GL3} &              \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] \\
  \midrule \texttt{K35} &             \cbox{1.0,0.7843137254901961,0.7843137254901961}{49.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.76s} &  [1.0] &  \cbox{0.8150711264898116,0.8150711264898116,0.9884659746251442}{0.95s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{55.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.56s} &  [1.0] &  \cbox{0.8815071126489812,0.8815071126489812,0.9635524798154556}{1.15s} &  [0.1] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{55.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.64s} &  [1.0] &  \cbox{0.8839677047289504,0.8839677047289504,0.9626297577854671}{1.34s} &  [0.1] \\
\midrule \texttt{L3132} &             \cbox{1.0,0.7843137254901961,0.7843137254901961}{26.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.59s} &  [0.1] &  \cbox{0.8667435601691656,0.8667435601691656,0.9690888119953864}{1.09s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{24.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.79s} &  [0.1] &  \cbox{0.8482891195693963,0.8482891195693963,0.9760092272202999}{1.28s} &  [0.1] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{24.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.77s} &  [0.1] &  \cbox{0.8421376393694733,0.8421376393694733,0.9783160322952711}{1.18s} &  [0.1] \\
         \texttt{L3133} &             \cbox{1.0,0.7843137254901961,0.7843137254901961}{38.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.94s} &  [0.1] &  \cbox{0.8815071126489812,0.8815071126489812,0.9635524798154556}{1.93s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{38.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.89s} &  [0.1] &   \cbox{0.9159554017685505,0.9159554017685505,0.950634371395617}{2.33s} &  [0.1] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{37.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.11s} &  [0.1] &    \cbox{0.849519415609381,0.849519415609381,0.9755478662053056}{1.79s} &  [0.1] \\
         \texttt{L3151} &            \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{15.12s} &  [0.1] & \cbox{0.8076893502499038,0.8076893502499038,0.9912341407151096}{17.94s} &  [0.1] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{12.74s} &  [0.1] & \cbox{0.9085736255286428,0.9085736255286428,0.9534025374855825}{31.74s} &  [0.1] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{18.03s} &  [0.1] & \cbox{0.8605920799692426,0.8605920799692426,0.9713956170703576}{31.69s} &  [0.1] \\
         \texttt{L3223} & \cbox{0.9889273356401385,0.813840830449827,0.813840830449827}{4.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.44s} &  [0.1] &  \cbox{0.8679738562091504,0.8679738562091504,0.9686274509803922}{0.92s} &  [0.1] &   \cbox{0.9889273356401385,0.813840830449827,0.813840830449827}{4.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.45s} &  [0.1] &    \cbox{0.875355632449058,0.875355632449058,0.9658592848904267}{0.98s} &  [0.1] &  \cbox{0.9870818915801615,0.8187620146097655,0.8187620146097655}{4.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.52s} &  [0.1] &  \cbox{0.9061130334486736,0.9061130334486736,0.9543252595155709}{1.26s} &  [0.1] \\
         \texttt{L3523} &            \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 7s} & [0.01] & \cbox{0.8618223760092272,0.8618223760092272,0.9709342560553633}{1m 59s} & [0.01] &              \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 2s} & [0.01] & \cbox{0.8532103037293348,0.8532103037293348,0.9741637831603229}{1m 44s} & [0.01] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{timeout} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{1m 9s} & [0.01] & \cbox{0.8384467512495194,0.8384467512495194,0.9797001153402537}{1m 44s} & [0.01] \\
  \midrule \texttt{TP3} &             \cbox{1.0,0.7843137254901961,0.7843137254901961}{1m 38s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{7.44s} &  [1.0] & \cbox{0.8335255670895809,0.8335255670895809,0.9815455594002307}{10.71s} & [10.0] &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{1m 40s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{7.63s} &  [1.0] & \cbox{0.8347558631295655,0.8347558631295655,0.9810841983852364}{11.09s} & [10.0] & \cbox{0.9953863898500577,0.7966166858900423,0.7966166858900423}{1m 44s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{11.45s} & [10.0] & \cbox{0.7892349096501345,0.7892349096501345,0.9981545559400231}{11.90s} & [10.0] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_nfccert_2pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize social welfare}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
\midrule \texttt{B2222} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] \\
         \texttt{B2322} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [0.01] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] \\
         \texttt{B2323} & \cbox{0.9423298731257209,0.9381007304882737,0.9381007304882737}{2.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.62s} &  [0.1] &  \cbox{0.7867743175701654,0.7867743175701654,0.9990772779700116}{0.63s} &  [0.1] &  \cbox{0.8790465205690119,0.8790465205690119,0.9644752018454441}{1.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.48s} &  [0.1] & \cbox{0.8359861591695501,0.8359861591695501,0.9806228373702423}{0.73s} &  [0.1] &  \cbox{0.9534025374855825,0.9085736255286428,0.9085736255286428}{2.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.14s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.18s} &  [0.1] \\
         \texttt{B2324} &  \cbox{0.895040369088812,0.895040369088812,0.9584775086505191}{11.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{4.88s} &  [0.1] & \cbox{0.8962706651287966,0.8962706651287966,0.9580161476355248}{11.06s} &  [0.1] &   \cbox{0.885198000768935,0.885198000768935,0.9621683967704728}{11.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{5.24s} &  [0.1] & \cbox{0.8704344482891195,0.8704344482891195,0.9677047289504037}{9.92s} &  [0.1] & \cbox{0.9695501730103806,0.8655132641291811,0.8655132641291811}{10.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.82s} & [0.01] & \cbox{0.8273740868896579,0.8273740868896579,0.9838523644752019}{2.51s} &  [1.0] \\
\midrule \texttt{S2122} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] \\
         \texttt{S2123} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [0.01] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] \\
         \texttt{S2133} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [0.1] \\
         \texttt{S2254} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{25.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.23s} & [0.01] &  \cbox{0.8802768166089965,0.8802768166089965,0.9640138408304498}{2.49s} & [0.01] & \cbox{0.9884659746251442,0.8150711264898116,0.8150711264898116}{24.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.02s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{3.02s} &  [0.1] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{28.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{1.32s} &  [0.1] &   \cbox{0.839677047289504,0.839677047289504,0.9792387543252595}{2.00s} & [0.01] \\
         \texttt{S2264} &               \cbox{1.0,0.7843137254901961,0.7843137254901961}{56.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{2.71s} &  [0.1] &  \cbox{0.8655132641291811,0.8655132641291811,0.9695501730103806}{4.93s} & [0.01] & \cbox{0.9870818915801615,0.8187620146097655,0.8187620146097655}{42.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{5.43s} &  [0.1] & \cbox{0.8163014225297962,0.8163014225297962,0.9880046136101499}{6.88s} & [0.01] &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{50.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{2.73s} &  [0.1] &   \cbox{0.823683198769704,0.823683198769704,0.9852364475201846}{3.65s} & [0.01] \\
 \midrule \texttt{RS212} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] \\
          \texttt{RS222} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] \\
          \texttt{RS213} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] \\
          \texttt{RS223} &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [0.01] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} &  [1.0] \\
\bottomrule
\end{tabular}


==> tables/detailed/comparison_nfccert_3pl.tex <==
\begin{tabular}[t]{l|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r|r|r@{\hskip1mm}r|r@{\hskip1mm}r}
\toprule
\multirow{2}{*}{\bf Game}
& \multicolumn{5}{c|}{\bf Maximize Player~1's utility}
& \multicolumn{5}{c|}{\bf Maximize Player~2's utility}
&  \multicolumn{5}{c}{\bf Maximize Player~3's utility}
\\
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c|}{Ours (PCFR$^+$)}
& LP & \multicolumn{2}{c|}{Ours (DCFR)} & \multicolumn{2}{c}{Ours (PCFR$^+$)}
\\
  \midrule \texttt{D32} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] \\
           \texttt{D33} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.06s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.06s} & [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} & [10.0] \\
  \midrule \texttt{GL3} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.01s} & [10.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] \\
  \midrule \texttt{K35} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  [1.0] \\
\midrule \texttt{L3132} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} & [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] \\
         \texttt{L3133} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [1.0] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} & [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.02s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [1.0] \\
         \texttt{L3151} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.08s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} & [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [0.1] \\
         \texttt{L3223} &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.03s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [0.1] &                \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.04s} & [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [0.1] &                 \cbox{0.7843137254901961,0.7843137254901961,1.0}{0.05s} &  [0.1] \\
         \texttt{L3523} & \cbox{0.8605920799692426,0.8605920799692426,0.9713956170703576}{13.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{7.41s} &  [0.1] &  \cbox{0.8741253364090734,0.8741253364090734,0.966320645905421}{14.31s} &  [0.1] & \cbox{0.8667435601691656,0.8667435601691656,0.9690888119953864}{15.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{8.17s} &  [0.1] & \cbox{0.8027681660899654,0.8027681660899654,0.9930795847750865}{9.36s} & [0.1] & \cbox{0.8482891195693963,0.8482891195693963,0.9760092272202999}{17.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{10.60s} & [0.01] & \cbox{0.8175317185697808,0.8175317185697808,0.9875432525951557}{13.52s} & [0.01] \\
  \midrule \texttt{TP3} &                \cbox{1.0,0.7843137254901961,0.7843137254901961}{47.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{4.56s} &  [1.0] & \cbox{0.8913494809688581,0.8913494809688581,0.9598615916955017}{10.06s} & [10.0] &     \cbox{0.9986159169550173,0.78800461361015,0.78800461361015}{48.00s} & \cbox{0.7843137254901961,0.7843137254901961,1.0}{4.97s} & [10.0] &  \cbox{0.8581314878892734,0.8581314878892734,0.972318339100346}{8.55s} & [1.0] & \cbox{0.9746251441753172,0.8519800076893502,0.8519800076893502}{45.00s} &  \cbox{0.7843137254901961,0.7843137254901961,1.0}{7.38s} & [10.0] &  \cbox{0.8163014225297962,0.8163014225297962,0.9880046136101499}{9.40s} &  [1.0] \\
\bottomrule
\end{tabular}


==> tables/eq_values_2players.tex <==
\sisetup{round-mode=places,round-precision=3,fixed-exponent=0,exponent-mode=fixed}
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrrr}
\toprule
\midrule
B2222 &     \num{0.28125} &      \num{0.09375} & \num{-4.75751704e-11} &   \num{-0.0267857143} &      \num{-0.3375} &       \num{-0.525} &  \num{-0.0307414105} &      \num{-0.3375} &       \num{-0.525} & \num{-0.187499989} &   \num{-0.562499632} & \num{-0.749894432} & \num{0.281249999} &      \num{0.09375} & \num{-2.92929601e-14} &   \num{-0.0267857143} &      \num{-0.3375} &       \num{-0.525} &   \num{-0.0267857144} &      \num{-0.3375} &       \num{-0.525} \\
B2322 & \num{0.180555556} & \num{0.0972222222} & \num{-1.24948804e-10} &   \num{-0.0429292929} & \num{-0.123015873} & \num{-0.317460317} &  \num{-0.0449760783} & \num{-0.123015873} & \num{-0.317460318} &         \unk &           \unk &         \unk & \num{0.180555555} & \num{0.0972222222} & \num{-6.36496335e-14} &   \num{-0.0429292929} & \num{-0.123015848} & \num{-0.317460318} &   \num{-0.0429292935} & \num{-0.123015873} & \num{-0.317460317} \\
B2323 &        \num{0.25} &  \num{0.124999995} & \num{-1.00825901e-09} & \num{-1.21844839e-11} &       \num{-0.125} & \num{-0.375000003} & \num{-0.00119617339} &       \num{-0.125} &       \num{-0.375} &         \unk &           \unk &         \unk &        \num{0.25} &  \num{0.124999995} & \num{-2.84601758e-09} & \num{-1.95539384e-09} & \num{-0.125000002} &       \num{-0.375} & \num{-5.66247296e-05} & \num{-0.125000001} & \num{-0.375022539} \\
B2324 & \num{0.305555544} &  \num{0.138888871} & \num{-7.25988977e-13} &            \unk &         \unk &         \unk &           \unk &         \unk &         \unk &         \unk &           \unk &         \unk & \num{0.305555555} &  \num{0.138888889} & \num{-5.92858037e-15} &            \unk &         \unk &         \unk &            \unk &         \unk &         \unk \\
S2122 &  \num{11.6363636} &   \num{5.99944896} &      \num{13.6363636} &      \num{7.65217392} &    \num{5.0432044} &    \num{9.5652196} &     \num{7.26213592} &   \num{3.84136858} &    \num{9.0776699} &   \num{0.81967214} &  \num{1.2836555e-11} &  \num{0.819672131} &        \num{50.0} &   \num{8.50763143} &            \num{50.0} &             \num{8.0} &   \num{5.19125683} &   \num{10.0000001} &      \num{8.00000001} &   \num{4.61102291} &         \num{10.0} \\
S2123 &  \num{11.6363636} &   \num{5.99944896} &      \num{13.6363636} &             \num{8.0} &   \num{5.19125683} &   \num{10.0000002} &     \num{8.00000001} &   \num{4.61102291} &         \num{10.0} &  \num{0.819672279} & \num{2.35586142e-12} &  \num{0.819672512} &        \num{50.0} &   \num{8.50763143} &            \num{50.0} &             \num{8.0} &   \num{5.19125683} &         \num{10.0} &      \num{8.00000001} &   \num{4.61102289} &         \num{10.0} \\
S2133 &  \num{15.1818182} &   \num{6.99236551} &      \num{18.1818182} &            \num{12.0} &   \num{6.55737705} &         \num{15.0} &     \num{12.0000001} &   \num{6.40746501} &         \num{15.0} &         \unk &           \unk &         \unk &        \num{50.0} &   \num{8.67126831} &            \num{50.0} &            \num{12.0} &   \num{6.55737705} &         \num{15.0} &            \num{12.0} &   \num{6.40746501} &         \num{15.0} \\
S2254 &  \num{23.5714284} &   \num{12.8302398} &      \num{28.5714286} &            \unk &         \unk &         \unk &           \unk &         \unk &         \unk &         \unk &           \unk &         \unk &       \num{100.0} &    \num{17.283507} &           \num{100.0} &      \num{20.0000001} &   \num{12.1900829} &   \num{25.0000001} &            \unk &         \unk &         \unk \\
S2264 &  \num{27.3333333} &   \num{13.8400652} &      \num{33.3333333} &            \unk &         \unk &         \unk &           \unk &         \unk &         \unk &         \unk &           \unk &         \unk &       \num{100.0} &   \num{17.4423662} &           \num{100.0} &            \unk &         \unk &         \unk &            \unk &         \unk &         \unk \\
 U212 &  \num{3.12333441} &    \num{3.1233344} &      \num{6.01020408} &      \num{3.07142857} &   \num{3.07142857} &   \num{6.01020408} &     \num{3.07142857} &   \num{3.07142857} &   \num{6.01020408} &   \num{3.18367347} &     \num{3.14285714} &   \num{6.17346932} &  \num{3.18367347} &   \num{3.17346938} &      \num{6.17346938} &      \num{3.18367347} &   \num{3.15884353} &   \num{6.17346939} &      \num{3.18367346} &   \num{3.14285713} &   \num{6.17346939} \\
 U213 &        \unk &         \unk &            \unk &            \unk &         \unk &         \unk &           \unk &         \unk &         \unk &   \num{5.16018028} &     \num{5.17078827} &    \num{9.5920461} &  \num{5.31632653} &   \num{5.42857143} &      \num{9.62244896} &      \num{5.20408163} &   \num{5.29756802} &   \num{9.62244898} &      \num{5.19616326} &    \num{5.2755102} &   \num{9.62244898} \\
 U222 &  \num{3.76489335} &   \num{3.76489335} &          \num{7.1875} &      \num{3.71874999} &      \num{3.71875} &   \num{7.17578125} &        \num{3.71875} &      \num{3.71875} &   \num{7.17578122} &    \num{4.0234375} &     \num{3.81152344} &      \num{7.59375} &   \num{4.0234375} &   \num{3.93014493} &         \num{7.59375} &       \num{4.0234375} &    \num{3.9048735} &      \num{7.59375} &       \num{4.0234375} &   \num{3.83854167} &      \num{7.59375} \\
 U223 &        \unk &         \unk &            \unk &            \unk &         \unk &         \unk &           \unk &         \unk &         \unk &   \num{6.53658639} &     \num{6.32645035} &   \num{11.4640564} &   \num{6.8671875} &   \num{6.78292854} &       \num{11.515625} &      \num{6.63141026} &   \num{6.58199411} &   \num{11.5130208} &      \num{6.57552083} &   \num{6.39843749} &   \num{11.4848958} \\
\bottomrule
\end{tabular}


==> tables/eq_values_3players.tex <==
\sisetup{round-mode=places,round-precision=3,fixed-exponent=0,exponent-mode=fixed}
\setlength{\tabcolsep}{2mm}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrr}
\toprule
\midrule
  \texttt{D32} &          \num{0.25} &  \num{0.249999999} &  \num{0.130872483} &          \num{0.25} &         \num{0.25} & \num{0} &          \num{0.25} &         \num{0.25} & \num{0.0} &         \num{0.25} &         \num{0.25} &  \num{0.041666666} &          \num{0.5} &        \num{0.25} &        \num{0.25} &         \num{0.25} &         \num{0.25} &        \num{0.25} & \num{0.249999994} &  \num{0.249999999} & \num{0.249999998} \\
  \texttt{D33} &    \num{0.42175765} &  \num{0.283950615} &  \num{0.239452522} &          \unk &         \unk &            \unk &          \unk &         \unk &            \unk &         \unk &         \unk &         \unk &  \num{0.580246913} & \num{0.296296296} & \num{0.283950617} &   \num{0.44444444} &  \num{0.296296296} & \num{0.283950617} & \num{0.432098765} &  \num{0.296296296} & \num{0.271604938} \\
  \midrule
  \texttt{GL3} &     \num{2.5048433} &    \num{2.5048433} &   \num{2.50484329} &    \num{2.47559839} &    \num{2.4755984} &      \num{2.47559838} &    \num{2.46748012} &   \num{2.46748013} &      \num{2.46748011} &         \unk &         \unk &         \unk &   \num{2.50484338} &  \num{2.50484338} &  \num{2.50484338} &   \num{2.50484331} &    \num{2.5048433} &  \num{2.50484333} &  \num{2.46748221} &   \num{2.46759256} &   \num{2.4676086} \\
  \midrule
  \texttt{K35} & \num{-0.0110262525} & \num{0.0169727412} & \num{0.0569116955} & \num{-0.0155917528} & \num{0.0149984651} &    \num{0.0523473338} & \num{-0.0159997753} & \num{0.0129084351} &    \num{0.0516608269} & \num{0.0220945918} & \num{0.0500643002} & \num{0.0882849236} & \num{0.0918532817} & \num{0.105952381} & \num{0.169234228} & \num{0.0918532818} & \num{0.0902832457} & \num{0.169234232} &   \num{0.0859009} & \num{0.0902430556} & \num{0.169234233} \\
  \midrule
\texttt{L3132} &   \num{0.570750119} &  \num{0.503563225} &  \num{0.605709586} &   \num{0.518758496} &         \unk &            \unk &   \num{0.467463991} &  \num{0.421642375} &            \unk &  \num{0.646482243} &  \num{0.618409656} &  \num{0.722801529} &  \num{0.853307142} & \num{0.778928568} & \num{0.802040265} &  \num{0.853307142} &  \num{0.778928568} & \num{0.802040263} & \num{0.853307142} &  \num{0.778928568} & \num{0.802040265} \\
\texttt{L3133} &   \num{0.419400186} &  \num{0.348393182} &  \num{0.415658193} &          \unk &         \unk &            \unk &          \unk &         \unk &            \unk &  \num{0.440808448} &  \num{0.458664164} &  \num{0.589900438} &  \num{0.645886884} & \num{0.654321878} & \num{0.708587624} &  \num{0.645886883} &  \num{0.654321878} & \num{0.708587624} & \num{0.645886884} &  \num{0.654321878} & \num{0.708587624} \\
\texttt{L3151} &          \unk &         \unk &         \unk &          \unk &         \unk &            \unk &          \unk &         \unk &            \unk &         \unk &         \unk &         \unk &  \num{0.179282208} & \num{0.197236749} & \num{0.222045455} &  \num{0.179282207} &  \num{0.182344838} & \num{0.222045451} & \num{0.171414873} &  \num{0.182344838} & \num{0.222045455} \\
\texttt{L3223} &     \num{1.0793883} &  \num{0.992182648} &   \num{1.14560401} &   \num{0.984159443} &  \num{0.959215648} &      \num{1.03291844} &   \num{0.887063033} &  \num{0.883073733} &     \num{0.860582363} &    \num{1.0114683} &  \num{0.915458148} &   \num{1.02002584} &   \num{1.37915528} &  \num{1.55591813} &  \num{1.45062178} &   \num{1.37915528} &   \num{1.55591813} &  \num{1.45062178} &  \num{1.37915528} &    \num{1.5559181} &  \num{1.45062178} \\
\texttt{L3523} &          \unk &         \unk &         \unk &          \unk &         \unk &            \unk &          \unk &         \unk &            \unk &         \unk &         \unk &         \unk &          \num{2.0} &         \num{2.0} &         \num{2.0} &         \unk &         \unk &        \unk &        \unk &         \unk &        \unk \\
\midrule
  \texttt{TP3} &    \num{1.46557341} &    \num{1.4765673} &   \num{1.03655203} &          \unk &         \unk &            \unk &          \unk &         \unk &            \unk &         \unk &         \unk &         \unk &   \num{1.73928442} &  \num{1.50592218} &    \num{1.083329} &         \unk &         \unk &        \unk &        \unk &         \unk &        \unk \\
\bottomrule
\end{tabular}


==> tables/game_size_summary.tex <==
\begin{tabular}{l|r|rrrrr}
    \toprule
    \textbf{Game} & \textbf{Nodes} & \textbf{NFCCE} & \textbf{EFCCE} & \textbf{EFCE} & \textbf{COMM} & \textbf{CERT}\\
    \midrule
        \texttt{B2222} & \num{1573} & \num{6915} & \num{21868} & \num{20534} & \num{65577} & \num{14638}\\
        \texttt{B2322} & \num{23839} & \num{89519} & \num{340619} & \num{503145} & \num{4090261} & \num{317180}\\
        \texttt{B2323} & \num{254239} & \num{1022286} & \num{5446015} & \num{7271972} & \unk & \num{4853180}\\
        \texttt{B2324} & \num{1420639} & \num{6397418} & \num{41633816} & \num{49264667} & \unk & \num{34920380}\\
    \midrule
        \texttt{D32} & \num{1017} & \num{33823} & \num{51593} & \num{536485} & \num{45070} & \num{9176}\\
        \texttt{D33} & \num{27622} & \num{11165451} & \num{71372690} & \unk & \num{10450812} & \num{520665}\\
    \midrule
        \texttt{GL3} & \num{7735} & \num{30021} & \num{37041} & \num{16950} & \num{547086} & \num{15234}\\
        \texttt{GL4} & \num{54310} & \num{207762} & \num{263850} & \num{129198} & \unk & \num{129336}\\
        \texttt{GL5} & \num{372883} & \num{1388727} & \num{1805331} & \num{937074} & \unk & \num{979674}\\
    \midrule
        \texttt{K35} & \num{1501} & \num{3592121} & \num{3826201} & \num{4535281} & \num{29235} & \num{6945}\\
    \midrule
        \texttt{L3132} & \num{8917} & \num{1222128} & \num{15329595} & \num{8400513} & \num{980190} & \num{96165}\\
        \texttt{L3133} & \num{12688} & \num{1500087} & \num{26166405} & \num{14519676} & \num{1095561} & \num{134604}\\
        \texttt{L3151} & \num{19981} & \num{34405970} & \unk & \unk & \num{5354895} & \num{217185}\\
        \texttt{L3223} & \num{15659} & \num{614847} & \num{5617510} & \num{4999142} & \num{4004046} & \num{273276}\\
        \texttt{L3523} & \num{1299005} & \num{58635336} & \unk & \unk & \unk & \num{51214448}\\
    \midrule
        \texttt{S2122} & \num{705} & \num{2903} & \num{7847} & \num{6227} & \num{12629} & \num{5465}\\
        \texttt{S2123} & \num{4269} & \num{19049} & \num{72377} & \num{52559} & \num{454565} & \num{49349}\\
        \texttt{S2133} & \num{9648} & \num{45931} & \num{171915} & \num{165859} & \num{2425875} & \num{139851}\\
        \texttt{S2254} & \num{712552} & \num{3758737} & \num{18655297} & \num{25303237} & \unk & \num{19348765}\\
        \texttt{S2264} & \num{1303177} & \num{7284509} & \num{34837769} & \unk & \unk & \num{40551631}\\
    \midrule
        \texttt{TP3} & \num{910737} & \num{7145312} & \num{11720048} & \num{6714256} & \unk & \num{10896416}\\
    \midrule
        \texttt{U212} & \num{598} & \num{15410} & \num{10604} & \num{9000} & \num{14338} & \num{768}\\
        \texttt{U213} & \num{6274} & \num{95194268} & \num{95250604} & \num{124453191} & \num{1638786} & \num{19160}\\
        \texttt{U222} & \num{734} & \num{55123} & \num{35047} & \num{32643} & \num{15914} & \num{952}\\
        \texttt{U223} & \num{6238} & \unk & \unk & \unk & \num{1184114} & \num{17776}\\
    \bottomrule
\end{tabular}

==> tables/steering-summary.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c}
      & Compute Then Steer  & Online Steer \\\toprule
     Full Feedback & $T^{-1/4}$ (\Cref{th:offline-then-steer}) & $T^{-1/6}$ (\Cref{th:online-steer}) \\\midrule
    Bandit & $T^{-1/8}$ (\Cref{th:bandit-offline-steer}) & {\em Open problem} \\ \bottomrule
    \end{tabular}
    \caption{A summary of the positive algorithmic results in \Cref{sec:decentralization}. In this table, we hide game-dependent constants and assume $\eps = T^{-1/2}$, since typical regret minimizers are capable of achieving this rate.}
    \label{tab:steering-summary}
    \vspace{-4mm}
\end{table}
